GibbsNet: Iterative Adversarial Inference for Deep Graphical Models

Directed latent variable models that formulate the joint distribution as $p(x,z) = p(z) p(x \mid z)$ have the advantage of fast and exact sampling. However, these models have the weakness of needing to specify $p(z)$, often with a simple fixed prior that limits the expressiveness of the model. Undirected latent variable models discard the requirement that $p(z)$ be specified with a prior, yet sampling from them generally requires an iterative procedure such as blocked Gibbs-sampling that may require many steps to draw samples from the joint distribution $p(x, z)$. We propose a novel approach to learning the joint distribution between the data and a latent code which uses an adversarially learned iterative procedure to gradually refine the joint distribution, $p(x, z)$, to better match with the data distribution on each step. GibbsNet is the best of both worlds both in theory and in practice. Achieving the speed and simplicity of a directed latent variable model, it is guaranteed (assuming the adversarial game reaches the virtual training criteria global minimum) to produce samples from $p(x, z)$ with only a few sampling iterations. Achieving the expressiveness and flexibility of an undirected latent variable model, GibbsNet does away with the need for an explicit $p(z)$ and has the ability to do attribute prediction, class-conditional generation, and joint image-attribute modeling in a single model which is not trained for any of these specific tasks. We show empirically that GibbsNet is able to learn a more complex $p(z)$ and show that this leads to improved inpainting and iterative refinement of $p(x, z)$ for dozens of steps and stable generation without collapse for thousands of steps, despite being trained on only a few steps.

==> figures/tikz/diagram.tex <==
\begin{tikzpicture}[
    black!50, text=black,
    font=\small,
    node distance=4mm,
    dnode/.style={
        align=center,
        % The shape:
        rectangle,minimum size=10mm,rounded corners,
        % The rest
        inner sep=5pt},
    rnode/.style={
        align=center,
        % The shape:
        rectangle,
        minimum width=30mm,
        minimum height=8mm,
        rounded corners,
        % The rest
        inner sep=3pt,
        very thick,draw=black!50},
    tuplenode/.style={
        align=center,
        % The shape:
        rectangle,minimum size=10mm,rounded corners,
        % The rest
        inner sep=5pt},
    darrow/.style={
        rounded corners,-latex,shorten <=5pt,shorten >=1pt,line width=2mm},
    mega thick/.style={line width=2pt}]

\matrix[row sep=18mm,column sep=5mm] {
    \node (z_0) [rnode,minimum width=20mm] {$ \zz_0 \sim \mathcal{N}(0,I) $}; &
    \node (z_i) [rnode] {$ \zz_i \sim q(\zz \, | \, \xx_{i - 1}) $}; &
    \node (xt_i) [rnode] {$ \xx_i \sim p(\xx \, | \, \zz_i) $}; \\


    \node (z_nm1) [rnode] {$ \zz_{N - 1} \sim q(\zz \, | \, \xx_{N - 2}) $}; &
    \node (xt_nm1) [rnode] {$ \xx_{N - 1} \sim p(\xx \, | \, \zz_{N - 1}) $}; &
    \node (z_n) [rnode] {$ \zz_N \sim q(\zz \, | \, \xx_{n - 1}) $}; &
    \node (xt_n) [rnode] {$ \xx_N \sim p(\xx \, | \, \zz_N) $}; \\
    
    \coordinate (dummy_0); &
    \node (zh_0) [rnode] {$ \hat{\zz} \sim q(\zz \, | \, \xx_{data}) $}; &
    \node (x_0) [rnode] {$ \xx_{data} \sim q(\xx) $}; &
    \coordinate (dummy_1); \\
};

\coordinate (fake_0_mid) at ($ (z_nm1.center)!0.5!(xt_nm1.center) $);
\coordinate (real_0_mid) at ($ (dummy_0)!0.5!(zh_0.center) $);
\coordinate (d_0_pos) at ($ (fake_0_mid)!0.5!(real_0_mid) $);

\node (D_0) at (d_0_pos) [dnode,left color=redfill,right color=greenfill] {$ D_1(\zz, \xx) $};

\coordinate (fake_1_mid) at ($ (z_n.center)!0.5!(xt_n.center) $);
\coordinate (real_1_mid) at ($ (x_0.center)!0.5!(dummy_1) $);
\coordinate (d_1_pos) at ($ (fake_1_mid)!0.5!(real_1_mid) $);

\node (D_1) at (d_1_pos) [dnode,left color=greenfill,right color=redfill] {$ D_2(\zz, \xx) $};

\begin{scope}[local bounding box=cycle_arrows]
    \draw[-latex,shorten <=1pt,shorten >=1pt,mega thick] (xt_i) to [bend left=45] (z_i);
    \draw[-latex,shorten <=1pt,shorten >=1pt,mega thick] (z_i) to [bend left=45] (xt_i);
\end{scope}

\begin{pgfonlayer}{background}
    \node (cycle) [fit=(xt_i) (z_i) (cycle_arrows),rnode,inner sep=5pt,draw=moreredfill,mega thick,dotted] {};
    \node (fake_0) [fit=(z_nm1) (xt_nm1),tuplenode,fill=redfill] {};
    \node (real_0) [fit=(zh_0) (x_0),tuplenode,fill=greenfill] {};
    \node (fake_1) [fit=(z_n) (xt_n),tuplenode,fill=redfill] {};
\end{pgfonlayer}

\node [below right=2pt of cycle.north west,text=myred!80!white] {\footnotesize Unclamped chain};
\node [below left=2pt of cycle.north east,text=myred!80!white] {\footnotesize $ i \in \{ 1, \ldots, N \} $};

\draw[-latex,shorten >=1pt,mega thick,dotted] (z_0) -- (cycle);
\draw[-latex,shorten >=1pt,mega thick] (x_0) -- (zh_0);

\draw[darrow,draw=redfill] (z_nm1) |- (D_0);
\draw[darrow,draw=greenfill] (zh_0) |- (D_0);

\draw[darrow,draw=redfill] (xt_n) |- (D_1);
\draw[darrow,draw=greenfill] (x_0) |- (D_1);

\draw[-latex,shorten <=35pt,shorten >=2pt,draw=moreredfill,dotted,mega thick] (z_i) -- node[pos=0.75,left=2mm,text=myred!80!white] {\scriptsize Take iteration $ N - 1 $} (fake_0.north);
\draw[-latex,shorten <=35pt,shorten >=2pt,moreredfill,dotted,mega thick] (xt_i) -- node[pos=0.75,right=2mm,text=myred!80!white] {\scriptsize Take iteration $ N $} (fake_1.north);

\end{tikzpicture}

